Combating catastrophic forgetting with developmental compression

Generally intelligent agents exhibit successful behavior across problems in several settings. Endemic in approaches to realize such intelligence in machines is catastrophic forgetting: sequential learning corrupts knowledge obtained earlier in the sequence, or tasks antagonistically compete for system resources. Methods for obviating catastrophic forgetting have sought to identify and preserve features of the system necessary to solve one problem when learning to solve another, or to enforce modularity such that minimally overlapping sub-functions contain task specific knowledge. While successful, both approaches scale poorly because they require larger architectures as the number of training instances grows, causing different parts of the system to specialize for separate subsets of the data. Here we present a method for addressing catastrophic forgetting called developmental compression. It exploits the mild impacts of developmental mutations to lessen adverse changes to previously-evolved capabilities and `compresses' specialized neural networks into a generalized one. In the absence of domain knowledge, developmental compression produces systems that avoid overt specialization, alleviating the need to engineer a bespoke system for every task permutation and suggesting better scalability than existing approaches. We validate this method on a robot control problem and hope to extend this approach to other machine learning domains in the future.

==> 04_results_fig_last_gen_fit.tex <==

\begin{figure}
\centering
\includegraphics[width=\linewidth]{Figures/Median_Min_SIG_FIG.png}
% \vspace{-1.5em}
\caption{\label{fig:last_gen_fit} Median Minimum Performance. Values computed across runs for the overall run champions in each. Mann-Whitney U test and Bonferroni correction applied to overall run champions reported here. All comparisons are significant (P < 0.0001).
}
\end{figure}




==> 04_results_table_evals.tex <==
\begin{table}
\caption{\label{table:results:evals} Total robot evaluations per run.}
% \vspace{-1.5em}
\begin{center}
\begin{tabular}{ | r || c | c | c | r | } \hline
		& Random 		& Control 		& Compression 	& Evals 			\\ 	\hline \hline 
E=2 	& 2x1500x100= 	& 2x1500x100= 	& 4x750x100= 	& $3 \times 10^5$	\\ 	\hline
E=3 	& 3x1500x100= 	& 3x1500x100= 	& 6x750x100= 	& $4.5 \times 10^5$ \\ 	\hline
E=4 	& 4x1500x100=	& 4x1500x100= 	& 8x750x100= 	& $6 \times 10^5$	\\ 	\hline
\end{tabular}
\end{center}
\end{table}
